Disentangling causal webs in the brain using functional Magnetic Resonance Imaging: A review of current approaches

In the past two decades, functional Magnetic Resonance Imaging has been used to relate neuronal network activity to cognitive processing and behaviour. Recently this approach has been augmented by algorithms that allow us to infer causal links between component populations of neuronal networks. Multiple inference procedures have been proposed to approach this research question but so far, each method has limitations when it comes to establishing whole-brain connectivity patterns. In this work, we discuss eight ways to infer causality in fMRI research: Bayesian Nets, Dynamical Causal Modelling, Granger Causality, Likelihood Ratios, LiNGAM, Patel's Tau, Structural Equation Modelling, and Transfer Entropy. We finish with formulating some recommendations for the future directions in this area.

==> LaminarAnalysis.tex <==
\subsection{Laminar analysis}
% Let's pose the idea
Lastly, \textit{laminar analysis} is a~new, neurophysiologically driven approach to causal inference from fMRI time series by means of measuring different histological layers of the cortex. Different types of information, commonly distinguished as feedforward and feedback, are associated with different histological layers. Therefore, a~laminar examination of the BOLD signal may reveal deeper insight in the directional and causal role of a~cortical region.

% What do layers represent?
The human cerebral cortex typically consists of six histological layers \citep{Brodmann1909}. The thalamus and Layer III from lower cortical areas are commonly implicated in sending feedforward information to Layer IV in higher cortical areas \citep{Jones1998} and to Layer V to a lesser extent \citep{Constantinople2013}. Feedback information is believed to be received by Layer II-III and V-VI \citep{Alitto2003}. %Layer I, closest to the surface, is thin and sparsely populated with neurons and will probably remain elusive to laminar fMRI.

Recently, the arterioles of layer II-III were indeed found to selectively dilate and increase their blood flow in the cat visual cortex depending on their orientation selective tuning curve \cite{OHerron2016}. In another study, the BOLD response was shown to have its onset in the input layer of rat motor and somatosensory cortex \cite{Yu2014}. These results suggest that the layer specific BOLD response contains information about the type and the directionality of information flow. This information may well be lost in standard fMRI experiments, in which the voxel size is approximately equal to the thickness of the cortex (\~3 millimeters \citep{Fischl2000}).

% Human fMRI layer advancements
Advancements in fMRI acquisition have made it possible to scan at submillimetre resolution, and promising layer specific results have been obtained in humans. Recently, deep layers of the primary visual cortex were found to activate in a feedback condition \citep{Kok2016}, although in a different experiment, the top layers were implicated in feedback processing \citep{Muckli2015}. Furthermore, in line with previous depth-dependent electrode recordings, the BOLD response that uniquely reflects trial by trial variance in the alpha and gamma bands was shown to be consistent with deep and middle layer origins of these oscillations \citep{Scheeringa2016}. This procedure has been tried outside the visual cortex as well: in the hippocampus and the entorhinal cortex, layer specific BOLD behaved according to neurophysiological expectation in an episodic memory task \citep{Maass2014}.

% Promising but not there yet
These results suggest human laminar BOLD signal may contain directional information. However, as this is a young area of research, it is in need of more validation and optimisation of the technique. Although progress is made in extracting a laminar signal, rigorous statistics has yet to be invented for routinely applying this to fMRI data \citep[][in submission]{VanMourik2017}. Hitherto, only single region laminar fMRI has been employed, but it may well be worthwhile to investigate how output layers of the one region influence the input layer of the other. 

